A Modular Graph-Native Query Optimization Framework

Complex Graph Patterns (CGPs), which combine pattern matching with relational operations, are widely used in real-world applications. Existing systems rely on monolithic architectures for CGPs, which restrict their ability to integrate multiple query languages and lack certain advanced optimization techniques. Therefore, to address these issues, we introduce GOpt, a modular graph-native query optimization framework with the following features: (1) support for queries in multiple query languages, (2) decoupling execution from specific graph systems, and (3) integration of advanced optimization techniques. Specifically, GOpt offers a high-level interface, GraphIrBuilder, for converting queries from various graph query languages into a unified intermediate representation (GIR), thereby streamlining the optimization process. It also provides a low-level interface, PhysicalSpec, enabling backends to register backend-specific physical operators and cost models. Moreover, GOpt employs a graph-native optimizer that encompasses extensive heuristic rules, an automatic type inference approach, and cost-based optimization techniques tailored for CGPs. Comprehensive experiments show that integrating GOpt significantly boosts performance, with Neo4j achieving an average speedup of 9.2 times (up to 48.6 times), and GraphsScope achieving an average speedup of 33.4 times (up to 78.7 times), on real-world datasets.

==> new-sec-intro-bak.tex <==
\section{Introduction}
\label{sec:intro}

Graph databases~\cite{neo4j,tigergraph,janusgraph,neptune,graphflow} have emerged as a powerful tool for maintaining and analyzing complex relationships in a myriad of domains.
At the heart of these databases lies graph pattern matching, a fundamental and extensively researched problem~\cite{lai2019distributed,aberger2017emptyheaded,ullmann1976algorithm,shang2008quicksi,yang2021huge, glogs,han13turbo,ammar2018distributed}.
Basic graph patterns (\bgps) matching aims at identifying all subgraphs in a data graph that match the given query pattern,
and is widely used in various areas~\cite{flake02www,hu18local,DBLP:journals/csur/CannataroGV10, prvzulj2006efficient,DBLP:journals/jcisd/ZhuYYLCCL05,gauzre15}.
%including but not limited to social network analysis\cite{flake02www,hu18local}, bioinformatics \cite{DBLP:journals/csur/CannataroGV10, prvzulj2006efficient}, and chemistry\cite{DBLP:journals/jcisd/ZhuYYLCCL05,gauzre15}.

Recently, there has been growing interest in complex graph patterns (\cgps) due to their utility in real-world applications. \cgps~ build upon \bgps~ by incorporating additional relational operations such as projection, selection, and aggregation, enabling more expressive and versatile query capabilities. %, and a range of graph query languages~\cite{cypher, angles17,pgql,gcore,gql,gsql,gremlin} support \cgps.
To enable efficient expression and execution of \cgps, existing graph databases typically adopt a coupled architecture
design, where the entire process is tightly integrated from query parsing to execution. These systems handle specific query languages, starting with a parser that translates the query into an internal representation.
A query optimizer then generates a physical execution plan, which is subsequently executed on an underlying execution engine.
Two representative examples of graph systems are Neo4j~\cite{neo4j} and \gs~\cite{graphscope}, illustrated in \reffig{example}.

Neo4j processes \cgps~written in Cypher query language~\cite{cypher}.
It employs a Cypher parser to convert the query into an intermediate structure. A \code{CypherPlanner} is then used to optimize
these queries using a combination of heuristic rules and cost-based optimization techniques. Finally, the optimized plans
are executed through Neo4j’s single-machine backend. In contrast, \gs~\cite{graphscope} is designed for industrial-scale
distributed graph processing. It supports \cgps~ expressed in Gremlin~\cite{gremlin}, utilizing a Gremlin parser to interpret the queries.
\gs~ utilizes a rule-based optimizer to refine the queries, distributing the execution of the optimized plans across its
dataflow-based distributed backend engine~\cite{qian2021gaia}.
%Below, we present examples of how \cgps~are processed and optimized in Neo4j~\cite{neo4j} and GraphScope~\cite{graphscope}, which serve as two representative graph systems.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.9\linewidth]{figures/new_motivation.pdf}
  \vspace*{-4.5mm}
  \caption{An Example of \cgps~in Neo4j and \gs}
  \label{fig:example}
\end{figure}

% \begin{example}
%   We illustrate an example of executing \cgps~in Neo4j and  \gs~in \reffig{example}.
%   Neo4j supports Cypher queries, by translating them into an internal format via its Cypher parser. Then, its query planner optimize it with heuristic rules like filter push down, and utilize cost-based optimization techniques to determine the optimal search order for the \bgp, as marked with the respective sequence numbers in the figure. Specifically, for cyclic patterns, Neo4j employs an \expandinto~to identify the edges that forms a cycle pattern. Lastly, Neo4j execute the query in its single machine backend.
%   In contrast, \gs~utilizes a Gremlin parser to support Gremlin queries, optimizing them through a rule-based optimizer. Like Neo4j, the optimizer rewrites the query plan by pushing down selection conditions, while adhering to the given expansion order. Specifically, it transforms the cyclic edge expansion, $e_3$ and $e_4$, into \wcoj, a distributed worst-case optimal join (abbr. wcoj)~\cite{ngo2018worst}, for efficient execution. Finally, \gs~executes the optimized plan in its distributed engines.
%   \eat{
%   Neo4j employs a Cypher parser to convert the Cypher query into an internal format first. Then, its query planner applies selection conditions ``\code{v1.id = \$id}'' and ``\code{e3.date > \$d}'' during pattern matching for $v_1$ and $e_3$.
%   It also determines the optimal search order for the matchings by expanding the edges in the sequence of $e_1$, $e_3$, $e_4$ and $e_2$, as marked with the respective sequence numbers in the figure. This order is chosen because the earlier expanded vertices and edges have filters, which help reduce the number of intermediate results.
%   When expanding $e_2$ lastly, the pattern becomes cyclic, and Neo4j employs an \expandinto~to identify the edges that connects the matchings for $v_1$ and $v_3$. Following pattern matching, Neo4j executes the remaining relational operations to aggregate the results and return the top 10 highest counts.
%   In contrast, \gs~utilizes a Gremlin parser to support Gremlin queries, optimizing them through a rule-based optimizer. Like Neo4j, the optimizer also rewrites the query plan by pushing down selection conditions, while adhering to the given expansion order.
%   After expanding $e_1$ and $e_2$, \gs~found that $e_3$ and $e_4$ targets to a common vertex $v_4$, creating a cyclic pattern.
%   In this case, \gs~transforms the expansion of $e_3$ and $e_4$ into a distributed worst-case optimal join (abbr. wcoj)~\cite{ngo2018worst}, denoted by a \wcoj. Specifically, this approach enables \gs~to directly intersect the result sets of $e_3$ and $e_4$ without flattening them, thereby identifying the common vertices, i.e., matchings of $v_4$.
%   Finally, similar to Neo4j, \gs~applies relational operations to the results following pattern matching.
%   }
% \end{example}

\stitle{Motivation and Challenges.}
The coupled architecture used by existing systems, such as Neo4j and \gs, for processing \cgps~poses two key limitations.
\eat{
The query processing is tightly integrated with the query languages, for example, Neo4j supports Cypher and \gs~ supports Gremlin only.
The optimization techniques are also closely tied to the underlying graph system, for example, Neo4j adopts \expandinto~and \gs~employs \wcoj~when matching cyclic patterns.
}

\etitle{Limitation 1}. In practice, while most graph systems are designed to support a single query language, there are scenarios where supporting multiple query languages becomes necessary to meet evolving user demands. For example, at \company~, users transitioning to \gs~ for scalable graph processing may require \gs~ to support Neo4j’s Cypher queries, despite \gs~ being originally designed for Gremlin. Moreover, the recent standardization of the graph query language GQL~\cite{gql} further motivates systems to gradually adapt and extend their capabilities.
However, until GQL achieves universal adoption, existing systems must maintain support for multiple query languages. This presents a significant challenge for existing systems due to their coupled architecture. For instance, \gs~is tightly integrated with a Gremlin parser and relies on a traversal-step-based intermediate representation, making it difficult to accommodate additional query languages.

\etitle{Limitation 2}. Different systems often employ distinct optimization strategies for \cgps, each with its strengths and limitations, while lacking certain advanced techniques available in others. For instance, Neo4j leverages cost-based optimization to determine the optimal search order for \cgps, as illustrated in \reffig{example} with the sequence numbers. However, Neo4j lacks advanced techniques like distributed worst-case optimal join~\cite{ngo2018worst}, which \gs~ employs for efficient cyclic pattern matching, marked as \wcoj in \reffig{example}. Conversely, \gs~relies on a rule-based optimizer that executes \cgps~ in a predefined search order, missing the sophisticated cost-based optimization strategies available in Neo4j.
Moreover, both systems lack support for recent advancements, such as high-order statistics proposed in~\cite{glogs}, which are critical for improving cardinality estimation and query planning. However, the tightly coupled architecture of these systems makes it difficult to seamlessly integrate such optimization techniques. % across platforms, further limiting interoperability and adaptability.

A potential solution to address the above limitations is to adopt a \emph{decoupled} and \emph{unified} optimization framework. This approach should offer several key features:
\begin{itemize}[leftmargin=1.2em, labelsep=0.5em]
  \item Support for multiple query languages: The framework must inherently support the parsing and processing of multiple query languages, enabling seamless interoperability and adaptability.
  \item Decoupling from existing systems: By being independent of specific graph systems, the framework can provide modular, layered programming interfaces that simplify integration with a wide range of platforms.
	\item Advanced optimization capabilities: The framework should integrate advanced optimization techniques from both academia and industry, consolidating them into a unified system to provide state-of-the-art optimization strategies.
\end{itemize}

Designing such a framework presents immediate challenges.


\etitle{\textbf{C1}: How to support cross-language compatibility?}
\cgps~ can be expressed in diverse query languages such as Cypher and Gremlin, each with distinct syntaxes and semantics. This diversity poses a significant challenge in integrating \cgps~ expressed in these languages into a unified framework.
%Existing systems are typically tailored to a single query language, limiting their flexibility. %Inspired by relational databases, some systems (\todo{add references}) have attempted to convert graph queries into a common intermediate representation, such as relational algebra. However, this approach often fails to exploit optimization opportunities specific to graph pattern matching~\cite{glogs,yang2021huge}, resulting in suboptimal performance for graph queries.
%Although some of them are planning to support the standardized graph query language GQL, it is still in the early stage.

\etitle{\textbf{C2:} How to exploit diverse optimization strategies?}
Different graph systems employ unique optimization strategies for \cgps, making it redundant and inefficient to re-implement advanced techniques across all systems. However, due to their tightly coupled designs, current graph systems like Neo4j and \gs~do not provide interfaces to seamlessly plug in optimization strategies from other systems.
An alternative approach is to convert graph operations in \cgps~ into their relational equivalents\cite{orientdb, DBLP:conf/sigmod/TianXZPTSKAP20, DBLP:conf/sigmod/SunFSKHX15}, enabling the use of well-established relational optimization techniques. While feasible, this \emph{non-graph-native} approach has limitations. It may miss optimization opportunities specific to graph pattern matching~\cite{glogs, yang2021huge}.%, and the additional step of translating optimized relational plans back into graph plans can lead to suboptimal performance.
Therefore, a more native and unified strategy is needed to integrate and share optimization techniques across graph systems effectively.
%Currently, there is a notable absence of a \emph{graph-native} optimization framework designed to holistically optimize \cgps,
%which not only requires to share the common optimization techniques but also accommodate diverse backend-specific optimization strategies.

\etitle{\textbf{C3:} How to effectively optimize \cgps?}
Optimizing \cgps~ is inherently a complex problem due to its multifaceted nature. One key challenge lies in the hybrid semantics of \cgps, which combine graph pattern matching with relational operations such as projection, selection, and aggregation. While existing graph optimization techniques\cite{yang2021huge, mhedhbi2019optimizing} are highly effective for \bgps, they often overlook the relational aspects.
Another challenge involves handling arbitrary type constraints. \cgps~ often include \bgps~ without explicit type constraints, where users have not assigned specific types on certain vertices and edges and can, in theory, match any type in the data graph. In practice, however, these elements are implicitly restricted by the data graph. Current graph optimization techniques~\cite{glogs} depend heavily on explicit type constraints, limiting their effectiveness in addressing \cgps~with arbitrary type constraints.



\eat{
  The issue of optimizing \cgps have multiple aspects:
  1. \cgps contain hybrid semantics of graph pattern matching and relational operations, while existing graph optimization techniques~\cite{glogs,yang2021huge,mhedhbi2019optimizing} typically just
  focus on the part of graph pattern matching; 2. \cgps often involve \bgps~without explicit type constraints, which in semantics means that the vertices (and edges) can potentially match any type in the data graph. However, this does not necessarily mean that these types are unrestricted, as the vertices and edges in the pattern are implicitly restricted by the underlying data graph, either through restrict schema definition (schema-strict)~\cite{graphscope, kuzudb} or the existing data~\cite{neo4j}.
  Existing graph optimization techniques~\cite{glogs, yang2021huge} rely heavily on explicit type constraints, posing limitations in handling \cgps~with arbitrary types.

However, existing graph systems like Neo4j and \gs~typically overlook the implicit type constraints, resulting in unnecessary intermediate results during query processing; 3. The optimization of \cgps~with arbitrary types remains challenging, as many existing graph optimization techniques~\cite{glogs, yang2021huge} rely heavily on explicit type constraints, posing limitations in handling \cgps~with arbitrary types.

The third challenge lies into  optimization of \cgps, which often involves \bgps~without explicit type constraints in practice, remains challenging.
A \bgp~without explicit type constraints does not imply a lack of constraints, as the vertices and edges in the pattern are implicitly restricted by the data graph's underlying schema.
However, graph systems like Neo4j and \gs~typically overlook the implicit type constraints, resulting in unnecessary intermediate results during query processing.
Moreover, Neo4j's schema-loose model that lacks a predefined schema, further complicates the inference of implicit constraints.
Additionally, many existing graph optimization techniques~\cite{glogs, yang2021huge} rely heavily on explicit type constraints, posing limitations in handling \cgps~with arbitrary types.
}

\eat{
\noindent\textbf{C1:} \textit{Cross-Language Compatibility.}
\cgps~can be expressed in various query languages such as Cypher and Gremlin.
A typical scenario arises when Neo4j users, who are familiar with Cypher, want to transition to \gs~for distributed graph processing.
However, \gs~currently only supports Gremlin, which features a query syntax that significantly differs from that of Cypher.
Moreover, the recently proposed GQL, a standardized graph query language by ISO~\cite{gql}, also requires support in \gs.
Unfortunately, \gs's coupled architecture design, which tailors intermediate representations specifically for Gremlin, poses challenges when trying to accommodate \cgps~expressed in other query languages like Cypher and GQL.
Other graph systems, typically designed for specific query language, encounter similar challenges.
\lourevise{[Not very related to optimizing CGPs].}
\lourevise{In practice, transferring data between databases to leverage the features of different databases is a common requirement.
A typical scenario arises when Neo4j users, who are familiar with Cypher, want to transition to \gs~for distributed graph processing, and \gs~currently only supports Gremlin.
Then, the common optimization strategies for \cgps~specifically implemented for Cypher and Neo4j's backend have to be reimplemented on \gs.
In general, it is unrealistic to implement a optimizer for \cgps~for every graph database, and it would involve a lot of redundant work.
Besides, a standardized graph query language named GQL is recently proposed by ISO~\cite{gql}, and it has the potential to become the widely accepted standard for graph languages in the future.
The future reusability further enhances the importance of the unified optimization framework for \cgps.}


\noindent\textbf{C2:} \textit{Various Advanced Optimization Strategies.}
The example illustrates various advanced optimization approaches used by different systems in managing \cgps.
Although both Neo4j and \gs~apply filter push down to reduce the intermediate results in \cgps, they differ in the way to handle \bgps~segment.
Specifically, Neo4j employs cost-based optimization techniques to determine the optimal search order for the \bgp, while \gs~relies solely on a rule-based optimizer.
In contrast\lourevise{[What does this mean]}, \gs~incorporates advanced techniques like a distributed worst-case optimal join algorithm for cyclic pattern matching, a capability that Neo4j currently lacks and instead utilizes an \expandinto~approach, which may face efficiency limitations.
Despite these advancements, the tightly coupled architecture of these systems poses challenges for the integration of sophisticated optimization techniques across different platforms.

\noindent\textbf{C3:} \textit{Arbitrary Type Constraints in \bgps.}
The core optimization of \cgps~lies in the \bgp~segment. However, \bgps~do not always feature explicit type constraints.
Nevertheless, the absence of explicit types in pattern does not always indicate a lack of constraints, since the vertices and edges in the pattern are implicitly restricted by the graph's underlying schema.
For instance, in \reffig{example}, $v_2$ lacks explicit type constraints, but it must be a \code{Person} because it is connected to \code{Person} $v_1$ by a \code{Knows} relationship.
Currently, \gs~executes queries using the exact specified types, without inferring implicit type constraints, which can lead to unnecessary intermediate results during pattern matching.
Neo4j operates similarly. Moreover, Neo4j employs a schema-loose model without a predefined schema, making it more difficult to infer implicit type constraints.
Meanwhile, \glogs, a graph system tailored for basic pattern matching, employs advanced optimization techniques like high-order statistics and hybrid join strategies, but is limited to \bgps~with explicit type constraints only, lacking support for arbitrary type constraints.
}

\stitle{Our Solutions.} To address the above limitations and challenges, we present \gopt, a unified optimization framework designed for \cgps, that can be integrated into existing graph systems to enhance their graph query capabilities. \gopt~introduces two essential features:

\etitle{\textbf{S1}: Decoupled System Design.}
\gopt~ enables cross-language compatibility through a unified intermediate representation (\ir) that encapsulates \cgps, combining \bgps~ and relational operations. To facilitate this, \gopt~ provides a high-level interface, \graphirbuilder, which translates queries from various graph query languages into the unified \ir. This design decouples query processing from specific query languages, allowing \gopt~ to support multiple languages seamlessly.
Additionally, \gopt~ introduces a low-level interface, \physicalbuilder, enabling graph systems to register their backend-specific operators. %For example, Neo4j can utilize \expandinto~ for its operations, while \gs~ can leverage \wcoj~ for cyclic edge expansions.
This flexibility allows \gopt~to integrate with various graph systems while maintaining compatibility with multiple query languages.
Currently, \gopt~supports both Cypher and Gremlin and has been successfully integrated into Neo4j and \gs. Note that the standardized GQL is not yet supported, as its official grammar interpretation tool (e.g., ANTLR~\cite{antlr}) has not been finalized.
 %demonstrating its adaptability and effectiveness in decoupling query processing from both query languages and system backends.

%, and currently \gopt~has already been integrated into Neo4j and \gs, respectively.

%Moreover, \gopt~features a physical representation that allows different systems to register their backend-specific operators, such as \expandinto~for Neo4j and \wcoj~for \gs~for cyclic edge expansions. Currently, \gopt~has been integrated into Neo4j and \gs, respectively.

%, which features a logical representation for high-level query semantics and a physical representation for low-level operator implementations.
%The logical representation decouples query processing from specific languages, and currently \gopt~supports both Cypher and Gremlin. Meanwhile, the physical representation allows

\etitle{\textbf{S2}: Graph-native Optimization for \cgps.}
Building on the unified \ir, \gopt~ enables graph-native optimization of \cgps~ by addressing the unique challenges posed by the interaction of \bgps~and relational operations. A comprehensive set of heuristic rules has been designed for the rule-based optimization process. These rules are extensible and pluggable, allowing them to be tailored for integration with different graph systems.
To handle \bgps~ with arbitrary types, we introduce an automatic type inference algorithm that deduces appropriate type constraints for vertices and edges in the pattern.
This algorithm leverages the underlying graph data and does not rely on schema-strict contexts, making it suitable for schema-loose systems like Neo4j~\cite{Angles_2023}. By inferring type constraints, we can apply cost-based optimization techniques, such as those in~\cite{glogs}, to enhance the accuracy of cardinality estimation using high-order statistics.
Using the estimated cardinalities, backend-specific physical operators, and their associated cost models, we propose a top-down search framework with branch-and-bound strategies to optimize \bgps. This framework determines the optimal execution plan by minimizing the estimated cost.
Moreover, the unified optimization framework allows advanced graph optimization techniques to be seamlessly integrated into the system. This ensures that any enhancements made to the framework are immediately beneficial to the integrated graph systems.

\eat{
\noindent\textbf{S1}: \textit{IR-based Query Processing for Cross-Language Compatibility.}
We utilize a unified intermediate representation (IR) to encapsulate \cgps~that blend \bgps~and relational operations. Leveraging this IR, \gopt~facilitates compatibility across various graph query languages by translating queries into this unified format \lourevise{and general optimizations for \cgps~can be easily implemented}. Currently, \gopt~supports both Cypher and Gremlin.

\noindent\textbf{S2}: \textit{Graph-native Optimization with Extensible Support for Diverse Backends.}
Based on the IR, we optimize \cgps~in a unified manner. We have designed a comprehensive set of heuristic rules that consider the interactions of \bgps~and relational operations in \cgp~(\refsec{rbo}), where the heuristic rules are extensible and pluggable to accommodate different graph systems.
For the \bgp~component, we have developed a cost-based optimization framework that enables different systems to register their own backend-specific physical operators~(\refsec{cbo}). For instance, when matching a cyclic pattern, \gopt~will adopt the \wcoj~for backend of \gs, while it will utilize an \expandinto~for Neo4j.
Based on this, we search for the optimal plan that minimizes the costs associated with backend-specific operators.

\noindent\textbf{S3}: \textit{Automatic Type Inference for Arbitrary Type Constraints.}
%To handle arbitrary type constraints in \bgps, we have developed three kinds of type constraints, \btype, \utype~and \unionall, to represent constraints for a single type, a union of multiple types, and all types within the data graph, respectively.
%Building upon this,
We introduce a type inference algorithm to automatically deduce the appropriate type constraints for vertices and edges in the pattern, leveraging the underlying schema.
Specifically, in schema-loose systems like Neo4j, we will carefully extract a comprehensive schema from the data graph prior to performing type inference
Furthermore, the inferred type constraints will further enhance the accuracy of cardinality estimation, thereby enhancing the effectiveness of cost-based optimization.

%With \gopt, we decouple query optimization from specific query languages, facilitating cross-language compatibility, while also separating optimization from underlying graph systems to seamlessly integrate advanced techniques across diverse platforms.
}

\stitle{Contributions}.
The main contributions of the paper are as follows:

\noindent(1) We have introduced \gopt, which as far as we know, stands as the first graph-native optimization framework for industrial-scale graph database systems.
\gopt~utilizes a unified intermediate representation to enable support for various graph query languages, and features an extensible optimization architecture to accommodate diverse backend systems.
This offers a holistic and unified approach to query optimization in complex real-life applications.

\noindent(2) We have engineered sophisticated algorithms to optimize \cgps.
Our approach incorporates a comprehensive set of optimization rules that explores the optimization potential between \bgps~and relational operations in \cgps.
For \bgps, we have devise an automatic type inference algorithm to deduce implicit type constraints, and introduce a novel cardinality estimation method that leverages these constraints.
Additionally, we allow backends to register their operator implementations and cost models to enhance the accuracy of cost estimation.
Building upon this, a cost-based optimizer has been developed with a top-down search framework and branch-and-bounding strategies.

\noindent(3) We have developed an open-source implementation of \gopt~ on top of Apache Calcite\cite{Begoli_2018}, leveraging Calcite’s relational optimization capabilities while incorporating our specialized graph-optimization techniques. The current implementation supports query languages Gremlin and Cypher, and integrates with graph systems Neo4j and \gs, enabling seamless interoperability and advanced optimization across diverse platforms.
The effectiveness of \gopt~ is validated through comprehensive experimental evaluations, showing significant performance improvements, with up to \todo{$xx\times$} speedup compared to state-of-the-art systems. Furthermore, \gopt~ has been successfully deployed with \gs~to handle real-world applications at \company, demonstrating its practicality, scalability, and ability to integrate into diverse environments effectively.


The paper is organized as follows: \refsec{background} covers background and challenges, \refsec{arch} provides an overview of the system architecture, \refsec{trans} describes intermediate representation and query transformation, \refsec{opt} details optimization techniques, \refsec{impl} discusses system implementation, \refsec{exp} presents experimental results, \refsec{rel} reviews related works, and \refsec{con} concludes the paper.


==> sec-intro.tex <==
\section{Introduction}
\label{sec:intro}

Graph databases~\cite{neo4j,tigergraph,janusgraph,neptune,graphflow} have emerged as a powerful tool for representing complex relationships in a myriad of domains.
At the heart of these databases lies graph pattern matching, a fundamental and extensively researched problem~\cite{lai2019distributed,aberger2017emptyheaded,ullmann1976algorithm,shang2008quicksi,yang2021huge, glogs,han13turbo,ammar2018distributed}.
Graph pattern matching aims at identifying all subgraphs in a data graph that matches the given query pattern,
and is widely used in various areas
including but not limited to social network analysis\cite{flake02www,hu18local}, bioinformatics \cite{DBLP:journals/csur/CannataroGV10, prvzulj2006efficient}, and chemistry\cite{DBLP:journals/jcisd/ZhuYYLCCL05,gauzre15}.

In real applications, there has been a growing interest in integrating graph and relational query semantics,
to support more complex queries~\cite{angles17,pgql,gcore,gql,gsql,gremlin}. %that involve both graph and relational operations
A typical query paradigm, termed as \patrel~in this paper, involves two parts:
first, identify subgraphs of interest through pattern matching,
and then perform relational operations such as projection and selection on the matched results for further analysis.
Below, we present an example of \patrel~with Cypher, a widely used graph query language.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.9\linewidth]{figures/new_example.pdf}
  \vspace*{-4.5mm}
  \caption{A Motivation Example}
  \label{fig:example}
\end{figure}

\begin{example}
% As depicted in \reffig{example}(a),
% we consider a graph database comprising vertex types of \code{Person}, \code{Product}, and \code{Place}, alongside specific edge types.
% \reffig{example}(b) showcases a \patrel. It begins by identifying a triangle pattern, which imposes a type constraint on vertex $v_3$ to be \code{Place}, as specified in the \code{MATCH} clause. Subsequent relational operations are then applied to the matched results, including filtering by place name and aggregating the data to return the top 10 entries, through \code{WHERE}, \code{COUNT}, \code{ORDER BY}, and \code{LIMIT} clauses.
% Note that in real applications,% such as fraud detection, 
% users might not be able to predetermine all feasible patterns with explicit type constraints assigned beforehand.
% Consequently, they often impose on the structure of the pattern, 
% without providing explicitly type constraints on every vertex or edge.
% Consequently, these untyped vertices and edges are treated as \emph{arbitrary}.
% % in real applications, users may not be able to specify all type constraints 
% %  that only $v_3$ is explicitly assigned a type constraint, while the other vertices and edges are not. Consequently, these untyped vertices and edges are treated as \emph{arbitrary}.
% \eat{
% However, this does not mean that the other vertices and edges in the query are without constraints. In reality, they are implicitly restricted by the graph's underlying schema. This notion is further clarified through examples we provide in \reffig{example}(c) and \reffig{example}(d), which illustrate valid and invalid type assignments, respectively.
% }
% %However, in real-world queries, such specificity is often not necessary. This is illustrated in \reffig{example}(c), where the query is constructed to detect any arbitrary triangle pattern in the graph, without specifying types for the vertices or edges involved.  %Following the identification of these patterns, the query then focuses on selecting the top 10 results from the grouped findings.
As depicted in \reffig{example}(a),
we consider a graph database comprising vertex types of \code{Person}, \code{Product}, and \code{Place}, alongside specific edge types.
\reffig{example}(b) showcases a \patrel. It begins by identifying a triangle pattern with a type constraint on vertex $v_3$ to be a \code{Place}, as specified in the \code{MATCH} clause. Subsequent relational operations are then applied to the matched results, including filtering by place name and aggregating the data to return the top 10 entries, through \code{WHERE}, \code{COUNT}, \code{ORDER BY}, and \code{LIMIT} clauses.
Note that users may not specify all feasible patterns with predefined type constraints.
Instead, they often establish constraints on pattern structure, e.g., a triangle pattern in this case,
without type constraints on every vertex or edge.
Thus, the untyped vertices and edges, such as $v_1$, $v_2$ and all edges in this example, are treated as with \emph{arbitrary types}.
\end{example}
\vspace*{-1mm}

\stitle{Motivation and Challenges.}
\eat{
From the above example, we can observe that \patrel~integrates a hybrid of graph and relational operations,
and one more consideration brought forth by real-world applications is that users may even express \patrel s in a variety of query languages,
such as Cypher\cite{cypher} and Gremlin\cite{gremlin}.
Furthermore, \patrel~facilitates the flexible descriptions of arbitrary patterns by
allowing flexible type constraints or no type constraints on vertices or edges in the patterns.
}
From the above example, we distill two primary features for \patrel:

\textbf{F1}: \hybrid. \patrel~melds graph pattern match with relational operations, showcasing a high level of expressiveness. This enables more nuanced and comprehensive data analysis by leveraging the strengths of both graph-specific functionalities and traditional relational data processing.

\textbf{F2}: \arbitrary. \patrel~allows arbitrary types for flexibility in pattern descriptions. This permits users to focus on the query application logic, liberating them from the monotonous task of specifying types for vertices and edges.

These features are prevalent not only in Cypher but also in most popular languages including Gremlin~\cite{gremlin}, GSQL~\cite{gsql}, G-Core~\cite{gcore}, PGQL~\cite{pgql}, and the standardized ISO/GQL~\cite{gql}.
Consequently, to develop an optimizer that speeds up \patrels, we immediately confront two significant challenges:

\textbf{C1}: \textit{How to optimize \patrel~in a unified framework?}
%
To address \hybrid in \patrel, a common approach is to convert graph operations into their relational equivalents~\cite{orientdb, DBLP:conf/sigmod/TianXZPTSKAP20, DBLP:conf/sigmod/SunFSKHX15},
allowing the use of established relational optimizers for the entire query. However, this \emph{non-graph-native} strategy might overlook more effective optimization possibilities for graph pattern matching~\cite{glogs}, leading to suboptimal execution plans.
Several academic works~\cite{glogs, aberger2017emptyheaded, lai2019distributed, yang2021huge} specifically focus on optimizing graph pattern matching, which could be directly applied to optimize the pattern part in \patrels, followed by the application of relational optimization techniques for the remaining relational operations. Yet, this segmented approach might not fully capture the interplay between the graph and relational segments of \patrels. %For instance, in \reffig{example}(b), the selection condition ``\code{v3.name = \$cityName}'' could be more efficiently integrated into the pattern matching process for $v_3$.
Graph databases, notably Neo4j~\cite{neo4j}, are sometimes observed to not fully leverage the latest advancements in graph optimization, which may result in suboptimal execution plans~\cite{glogs}.
Currently, there is a notable absence of a graph-native optimization framework designed to holistically optimize \patrels, which would ideally apply graph-specific techniques to the graph part in the query and relational techniques to the relational segment, while also considering the interactions between these two components.

\textbf{C2}: \textit{How to handle Arbitrary Types in \patrel?}
%
Matching vertices and edges in patterns designated as \arbitrary can potentially be more costly compared to those with explicit type constraints. Nevertheless, the absence of explicit types in pattern does not always indicate a lack of constraints,
since the vertices and edges in the pattern are implicitly restricted by the graph's underlying schema.
This is exemplified in \reffig{example}(c), where two valid type assignments are demonstrated. Conversely, the type assignment in \reffig{example}(d) is not valid. In this instance, $v_1$ is typed as a \code{Product} and $v_2$ as a \code{Place}, yet there is no suitable type of edge to connect $v_2$ to the known \code{Place} vertex $v_3$.
Overlooking the implicit constraints in a query can lead to significant computational wastage, while mishandling them poses the risk of producing inaccurate results. Current graph optimization techniques~\cite{glogs,yang2021huge} often require explicit types for optimization, with limitations in handling \arbitrary in \patrels.
%Therefore, it is crucial to consider the implicit type constraints when optimizing arbitrary patterns.


\stitle{Our Solutions.}
To address the above challenges, we propose \gopt, a graph-native optimization framework for \patrels.
%This framework is characterized by the following innovative features: % that aim to enhance performance of executing \patrel:
It is characterized by three innovative features:

\textbf{S1}: \textit{A Unified Intermediate Representation}.
To effectively represent \patrel~that combine graph and relational operations, we have established a unified query representation. This approach effectively merges expressions from both graph and relational domains, enabling a cohesive process for \patrels. The unified expression layer not only streamlines the optimization process, but also ensures that \gopt can translate various query languages into this unified format, to guarantee cross-query-language compatibility. Currently, we have already supported Cypher and Gremlin in \gopt.

\textbf{S2}: \textit{Automatic Type Inference for Arbitrary Types}.
%\gopt~ effectively incorporates the ability to handle \arbitrary in \patrels.
Following the proposal of schema for property graph~\cite{Angles_2023}, we have developed three type constraints of
\btype, \utype~and \unionall, as detailed in \refsec{patrel}, to represent constraints for a single type, a union of multiple types, and all types within the graph schema, respectively.
Building upon this, we introduce a type inference algorithm to automatically deduce the appropriate type constraints for vertices and edges from \arbitrary~in the pattern.

\textbf{S3}: \textit{Graph-native Optimization}.
With the IR in place, \gopt is poised to implement heuristic optimization rules.
These include relational rules like \trimrule, graph rules such as \fusionrule, and relational-graph interplay rules
including \filterrule~and {\commonrule~}(\refsec{rbo}).
Additionally, \gopt~ draws on the state-of-the-art graph optimization techniques, including leveraging high-order statistics~\cite{glogs} and utilizing the distributed worst-case-optimal join (abbr.~wcoj) algorithm~\cite{ammar2018distributed}
for optimizing pattern matching in \patrel. 
Note that applying these advanced techniques is challenging, particularly in the context of dealing with \arbitrary (\refsec{cbo}).

% (2) \textit{Type Extensibility}:
% Beyond supporting the conventional \btype,
% \gopt~ incorporates the capability to accommodate \utype~ and \unionall,
% allowing for the representation of arbitrary types within user-given queries.
% In addition, we design a type inference algorithm to deduce and validate \unionall,
% that try to fills in the necessary type details for it.
% This allows great flexibility in the express of \patrel~while not compromising the optimizations for \upattern.

% (3) \textit{A Novel Graph Optimizer for \upattern}:
% To optimize \upattern, rather than relying on an exhaustive enumeration and optimization for all \bpatterns,
% \gopt~ employs a top-down framework with branch-and-bounding strategies, to identify the optimal plan for \upattern direclty.
% Specifically, it utilizes a novel approach for estimating the cardinality of \utype~ and therefore \upattern,
% to efficiently approximate the cost needed to execute a \upattern.

% (4) \textit{Integration with Apache Calcite\cite{Begoli_2018} for Relational Optimization}:
% \gopt~ is seamlessly integrated into Apache Calcite\cite{Begoli_2018},
% a widely adopted open-source framework for query optimization.
% This integration allows \gopt~ to benefit from the existing techniques for relational optimization.

%\stitle{Contributions.}
The main contributions of this paper are as follows:

(1) We have introduced \gopt, which as far as we know, stands as the first graph-native optimization framework for industrial-scale graph database systems. \gopt is distinguished by its Intermediate Representation abstraction, enabling the effective optimization of \patrels~across various graph query languages. This framework adeptly integrates both graph and relational operations, offering a holistic and unified approach to query optimization in complex real-life applications.

(2) We have engineered sophisticated algorithms to process and optimize \textit{arbitrary patterns}. Our approach includes an efficient method for type inference, to deduce implicit type constrains from \arbitrary. We also incorporate a comprehensive set of optimization rules, meticulously crafted to consider the hybrid nature of these queries. Moreover, we have pioneered a novel cardinality estimation method that takes \arbitrary into account. Building upon this, a cost-based optimizer has been developed, operating in a top-down framework with branch-and-bounding strategies.

(3) We have implemented \gopt atop the open-source optimization framework Apache Calcite~\cite{Begoli_2018}, {leveraging its relational optimization capabilities and integrating our specialized graph-optimization techniques}.
%inheriting its capabilities for optimizing relational operations. This integration has been smoothly executed to include our specialized graph-optimization techniques. 
The effectiveness of our proposed techniques is validated through comprehensive experimental evaluations, demonstrating significant performance improvements with up to $389\times$ speedup compared to state-of-the-art systems.
Additionally, \gopt has been successfully deployed in real applications in Alibaba Group, demonstrating its practicality and scalability.

% We organize the paper as follows. We present the background and challenges in \refsec{background}.
% An overview of the system architecture is provided \refsec{arch}.
% The process of query transformation and the methodology for type inference are described in \refsec{trans},
% followed by the optimization techniques in \refsec{opt}.
% The system implementation details are presented in \refsec{impl}.
% We present the experimental results in \refsec{exp}.
% Lastly, we discuss related works in \refsec{rel}, and conclude the paper in \refsec{con}.
The paper is organized as follows: \refsec{background} covers background and challenges, \refsec{arch} provides an overview of the system architecture, \refsec{trans} describes query transformation and type inference, \refsec{opt} details optimization techniques, \refsec{impl} discusses system implementation, \refsec{exp} presents experimental results, \refsec{rel} reviews related works, and \refsec{con} concludes the paper.

==> sec-pre.tex <==
\section{Preliminaries}
\label{sec:pre}
We present some preliminaries of \patrel~ optimization problem in this section,
including the intermediate representation for \patrel,
and the cost model based on the unified abstraction.

\subsection{Cost Model}
With the DAG serving as a standardized foundation for representing \patrel, 
we are equipped to devise a cost model that can estimate the execution cost associated with the query plan. 
The cost model takes two aspects into account:
The first part is the number of intermediate results generated during execution, 
which represents the communication cost in a distributed environment. 
This cost arises due to the need to fetch intermediate results from one machine to another for further processing, 
and a large volume of intermediate results can significantly impact network traffic and overall query performance.
The second part is the cost of the operators in DAG, that represents the computational cost,
and is defined by the individual processing expenses associated with the different operators in the set $\Omega$.
For graph operators, the cost is mainly determined by the number of graph elements that are processed by the operator,
and we will discuss the details later.
For relational operators, we follow the common operator cost definition used in RDBMS.
By taking both the communication and computation costs into consideration, 
the cost model is utilized to evaluate the execution cost of the query plan.

Based on the IR abstraction and cost model, we propose the problem statement of \textit{\patrel~ Optimization}:

\stitle{Problem Statement}: 
Given a \patrel~ $Q$, that would be firsly translated into a query plan based on the IR abstraction,
the goal of \textit{\patrel~ Optimization} is to find an optimal query plan $Plan^*$,
such that the execution cost of $Plan^*$, computed based on the cost model, is minimized.

In the following, we provide an overview of the system architecture in \refsec{arch}. 
Following that, we describe the process of transforming a user-provided query into a unified logical plan, 
and the methodology for type inference and validation in \refsec{trans}. 
Afterward, we delve into the optimization techniques in \refsec{opt}, including the rule-based optimization and cost-based optimization,
along with the details of the system implementation in \refsec{impl}
Lastly, we will present the experimental results in \refsec{exp}.

==> sec-rel.tex <==
\vspace*{-1mm}
\section{Related Works}
\label{sec:rel}
\vspace*{-1mm}

\stitle{Graph Query Languages.}
Numerous graph query languages have been developed for querying property graphs\cite{property_graph}. Gremlin \cite{gremlin} represents graph traversal as a sequence of steps, {each offering functions such as navigating through graph vertices and edges}. % or retrieving their properties.
{Cypher \cite{cypher} crafted for Neo4j \cite{neo4j}, 
%stands out as one of the most prevalent graph query languages in academic and industry settings,
allows users to describe graph patterns with an ASCII-art syntax while integrating relational operators similar to those 
%found 
in SQL}. %G-Core \cite{gcore}, bearing resemblance to Cypher in syntax, strides towards composability where both the input and output of queries are graphs.
%Similarly, PGQL \cite{pgql} adheres to the SQL paradigm, extending it with capabilities for graph pattern matching, path finding, and reachability queries. GSQL \cite{gsql}, designed for TigerGraph \cite{tigergraph}, supports user-defined functions and procedures, enabling complex graph workloads that go beyond pattern matching ({e.g., PageRank and SSSP}).
%, including algorithms like PageRank and SSSP.
The recently published GQL \cite{gql} is a new standard developed by ISO committee for querying property graphs, with a consensus effort that integrates previous advancements.
{More typical graph query languages like G-Core \cite{gcore}, PGQL \cite{pgql} and GSQL \cite{gsql} are not discussed here due to space constraints.}
{While these languages focus on querying property graphs, SPARQL \cite{sparql} is a W3C recommendation for querying Resource Description Framework (RDF) graphs \cite{rdf}.}
Despite the proliferation of these graph query languages, there remains a notable gap: the lack of a dedicated graph optimizer designed to enhance the efficiency of queries written in these languages.

\stitle{Graph Query Optimization.}
{Graph pattern matching is fundamental in graph query processing, with subgraph isomorphism \cite{ullmann1976algorithm} being widely recognized as the most prevalent semantics.}
%Graph pattern matching is a fundamental problem in graph query processing and has been studied in numerous works. Subgraph isomorphism \cite{ullmann1976algorithm} is widely recognized as the most prevalent semantics for graph pattern matching. 
In a sequential context, Ullmann's introduction of the first backtracking algorithm \cite{ullmann1976algorithm} marked a significant advancement in graph pattern matching. This has led to various optimizations, including tree indexing \cite{shang2008quicksi}, symmetry breaking \cite{han13turbo}, and compression techniques \cite{bi2016efficient}. 
Due to the challenges in parallelizing backtracking algorithms, join-based algorithms have been developed for distributed environments. These algorithms often hinge on cost estimation to optimize join order for matching patterns efficiently. For instance, binary-join algorithms \cite{lai2015scalable, lai2019distributed} estimate costs using random graph models. In contrast, the work in \cite{ammar2018distributed} adopts the \wcoj~algorithm \cite{ngo2018worst}, ensuring a cost that remains within a worst-case upper bound. 
{Recognizing the limitations of both binary join and \wcoj~methods in consistently delivering optimal performance~\cite{lai2019distributed}, researchers have turned to hybrid approaches \cite{aberger2017emptyheaded, mhedhbi2019optimizing, yang2021huge} that adaptively select between binary and \wcoj~techniques based on the estimated costs.}
%Recognizing the limitations of both binary join and {wcoj} methods in consistently delivering optimal performance~\cite{lai2019distributed}, researchers have turned to hybrid approaches \cite{aberger2017emptyheaded, mhedhbi2019optimizing, yang2021huge}. These approaches aim to adaptively select between binary and {wcoj} techniques based on which method incurs lower costs in a given situation.
For more accurate cost estimation, \cite{mhedhbi2019optimizing} and \cite{glogs} suggested to leverage high-order statistics.
%To further enhance cost estimation, the authors in \cite{mhedhbi2019optimizing} and \cite{glogs} have suggested leveraging high-order statistics to compute more effective execution plans for graph pattern matching.
While these studies have significantly improved graph pattern matching, they are not designed to address graph queries in practice that often encompasses relational operations. %their applicability is predominantly confined to that specific context. %They are not designed to address the broader spectrum of graph queries, which often encompass relational operations such as aggregation and projection.

{
For optimizing queries on RDF graphs, \cite{DBLP:conf/edbt/TsialiamanisSFCB12} outlines several heuristic rules designed to enhance SPARQL query optimizers, 
\cite{DBLP:conf/www/StockerSBKR08, DBLP:conf/edbt/RabbaniLH21, 7930124} propose cost-based optimization techniques based on cardinality estimation and join reordering, 
and \cite{DBLP:conf/edbt/YakovetsGG15} delves into optimizing regular path queries (RPQs) by utilizing fixpoint evaluation for property paths.
This work focuses on query optimizations on property graph databases.
}

\stitle{Graph Queries Over Relational Database.}
The practice of modeling and querying graphs in the context of relational databases has an extensive history \cite{guting_vldb94}.
GraphiQL \cite{jindal14} was designed as a graph query language to facilitate the expression of graph analytics over relational data. Noticing the inefficiency of translating pattern matching queries into single SQL queries, {the study in \cite{osti_924192} aims to generate multiple SQL statements specifically for graph pattern matching}. %, achieving a significant improvement in performance.
{The work in \cite{jachiet20} extends relational algebra with a fixed-point operator, enhancing optimization for recursive queries common in graph data structures}.
%The work in \cite{jachiet20} proposes an extension to the standard relational algebra by incorporating a fixed-point operator. This addition is particularly adept at optimizing recursive queries, which are commonly encountered in graph data structures.
Meanwhile, the authors of \cite{sun_2015} suggest an approach that combines relational storage for adjacency information with JSON storage for vertex and edge attributes, enabling the direct utilization of relational optimizers in graph query processing.
Going beyond high-level languages, the research in \cite{graphgen2017} explores the idea of defining graphs as transformations over underlying relational datasets, effectively creating graph views.
GRFusion \cite{hassan18}, implemented atop a relational database system, executes cross-data-model query plans that amalgamate traditional relational operators with newly introduced graph operators, offering a versatile query processing framework.
The study in \cite{jin2022} takes an approach by defining specific graph operations like retrieving neighbors from a vertex, as predefined joins in a relational database. This method identifies optimization opportunities within relational queries, leveraging these predefined joins to expedite execution. In this study, we focus on optimizing graph queries specifically for graph-native databases, encompassing unique topics such as union types~\cite{Angles_2023} that have not been thoroughly explored in the realm of relational databases.


%\stitle{Graph Databases And Systems.}


